Identifiability of AMP chain graph models

We study identifiability of Andersson-Madigan-Perlman (AMP) chain graph models, which are a common generalization of linear structural equation models and Gaussian graphical models. AMP models are described by DAGs on chain components which themselves are undirected graphs. For a known chain component decomposition, we show that the DAG on the chain components is identifiable if the determinants of the residual covariance matrices of the chain components are monotone non-decreasing in topological order. This condition extends the equal variance identifiability criterion for Bayes nets, and it can be generalized from determinants to any super-additive function on positive semidefinite matrices. When the component decomposition is unknown, we describe conditions that allow recovery of the full structure using a polynomial time algorithm based on submodular function minimization. We also conduct experiments comparing our algorithm's performance against existing baselines.

==> major/algo.tex <==
\section{Algorithm}
The main idea of our top-down algorithm is outlined in 

\ignore{
\begin{figure*}
\centering
  \begin{subfigure}{0.22\textwidth}
    \includegraphics[width=1.35\textwidth]{fig/01234.png}
      \caption*{$G_1:0-1-[2,3]-4$}
      \label{fig:exp_a} 
  \end{subfigure}
  \hspace{8mm}
  \begin{subfigure}{0.22\textwidth}
    \includegraphics[width=1.35\textwidth]{fig/01342.png}
      \caption*{$G_2:0-1-2-[3,4]$}
      \label{fig:exp_b} 
  \end{subfigure}
  \hspace{8mm}
  \begin{subfigure}{0.22\textwidth}
    \includegraphics[width=1.35\textwidth]{fig/02314.png}
      \caption*{$G_2:0-[2,3]-1-4$}
      \label{fig:exp_c} 
  \end{subfigure}
\caption{Chain graph experiments
\label{fig:chain_graph}
}
\vskip -0.3cm
\label{fig:algorithm}
\end{figure*}
}

